STraM: A strategic network design model for national freight transport decarbonization

National freight transport models are valuable tools for assessing the impact of various policies and investments on achieving decarbonization targets under different future scenarios. However, these models struggle to address several critical elements necessary for strategic planning, such as the development and adoption of new fuel technologies over time, inertia in transport fleets, and uncertainty surrounding future transport costs. In this paper, we develop a strategic network design model, named STraM, that explicitly incorporates these key factors. STraM provides a network design plan that includes infrastructure investments and fuel technology decisions, aiming to achieve cost-effective decarbonization of the freight transport system. The model's output can be used as input for higher-resolution national freight transport models to yield results with greater operational detail. We demonstrate the application of STraM through a case study of Norway, offering valuable insights into the strategic planning of sustainable freight transport.

==> Notes/introduction.tex <==

\red{
Thoughts:
\begin{itemize}
    \item Quotes from \cite{deJong2004NationalDevelopment}: ``For future development of national and interntaional fregith transport models, we reocmmend building an integrated family of mutually consistent models at two levels of resolution: (1) a detailed (high resolution) set of models and \textbf{(2) a fast (low resolution) policy analysis model}. (...) The family of several models should satisfy the principle of \textbf{Occam's razor: each model is the simplest model for the desired purpose, but not simpler} (page 114---115)
    \begin{itemize}
        \item These quotes help motivate our simple approach for strategic planning
        \item Similar quote found on page 246 of ``Modelling Freight Transport'' by Tavasszy and De Jong.
    \end{itemize}
    \item Current practice in the literature (using deterministic models) is scenario analysis: test effect of certain policy measures in different settings. Perhaps refer to Stein Wallace to argue that this is no good for strategic decision making under uncertainty. \notesjb{Note that the current practice currently is both static and deterministic. Start with the static-dynamic argument, then deterministic (scenario analysis)-stochastic.}
    \item \notesjb{Great setup for the structure Ruben. I feel like this will work :) }
\end{itemize}
}

\pt{Initial motivation: decarbonization \red{in general}}
\ppt{\red{For example, in Norway ...}}
\ppt{Emission targets: ...\% by 2030, 2050 (check numbers)\orange{ Note that Ireland has as a target only 60\% reductions according to \citet{Yan2021Climate2050}}}
\ppt{Important contributor: (freight) transport. Increasing share in the future (hard-to-abate)}
\ppt{Some statistics on emissions of (freight) transport}
\ppt{Need to decarbonize freight transport}
\ppt{\notesjb{\color{black}How to decarbonize? Cite \cite{Kaack2018DecarbonizingShift}. Maybe make some changes to the list.
\begin{itemize}
    \item reducing the demand for freight transport
    \item optimizing vehicle use and loading
    \item increasing the efficiency of freight vehicles
    \item reducing the carbon content of fuel used to transport freight
    \item  shifting freight to low carbon-intensity modes
\end{itemize}}}


\pt{This paper: develop a framework for strategic national freight transport modeling that can help national governments determine how to decarbonize freight transport sector. Should help specific questions:}
\ppt{What (new) technologies should be used/are attractive?}
\ppt{What associated infrastructure investments are needed?}
\ppt{(more subquestions?)}
\ppt{\notesjb{What kind of emission reduction trajectories/pathways can be achieved in freight transport? E.g. is $85\%$ emission reduction feasible?} (Quote from \citet{Yan2021Climate2050}: \textit{"There is a need to quantitatively explore pathways to achieve low emission freight transport and to inform future policy development"})}


\pt{In the literature, national freight transport models have been developed}
\ppt{Numerous models exist \notesjb{See tables in the reviews from \citep{deJong2004NationalDevelopment,deJong2013RecentEurope}}}
\ppt{Used for policy advice, ... and more...
\begin{itemize}
    \item \notesjb{\citet{deJong2013RecentEurope}: "Freight transport models are used to assess the \textbf{impacts} of different types of policy measures, such as changes in national regulations and taxes or infrastructure investments in \textbf{specific links, nodes and corridors}"}
\end{itemize}
}
\ppt{Most approaches based on four-step procedure. First two steps: generate OD-matrix; last two steps: assign demand to modes and routes. \notesjb{I agree that we can use this, but, there are also some references that state that this is somewhat outdated. \citet{deJong2016TheLevel}: "In recent years, many national freight transport models have changed considerably, moving away from the four-stage model that was originally developed for passenger transport, especially by including more aspects of transport logistics and sometimes even inventory logistics."}}
\ppt{(what else to mention here?)}
\ppt{\notesjb{Maybe we (very) briefly introduce tactical and strategic network design problems, but then quickly move the focus to (inter-)national freight transport models.
\begin{itemize}
    \item (service) network design \textbf{reviews}: \cite{Crainic2000ServiceTransportation, Steadieseifi2014MultimodalReview}
    \item When targeting stochasticity, cite \cite{Demir2016AUncertainty} who investigates both uncertainty in demand and travel time. \red{(yes, but note this is \textit{operational} uncertainty, we are interested in \textit{strategic} uncertainty; we should emphasize this difference somewhere)}
\end{itemize}
}}


\pt{Recent trend towards more and more detailed (modular) models}
\ppt{(mention logistics modules here). }
\orange{
\begin{itemize}
    \item \citet{deJong2013RecentEurope}:
    \begin{itemize}
    \item \textbf{\color{black}"The logistics models that have been developed up to this point concentrate on the linkbetween  trade  flows  (of  commodities)  and  physical  transport  flows  (of  vehicles). "}
    \item "The road ahead": list of expansions all going into more details.
    \item "the  current  paper  discusses  in particular  efforts  to  include  elements  of  logistics  decision  making  in  national  and  international freight transport models, since we consider that this has been the most important recent trend in freight transport modelling at that spatial level."
    \item The SMILE model (later SMILE?, see Tavasszy et al.1998and Bovenkerk2005) has been  the  Dutch  national  freight  model  system  for  over  a  decade.  SMILE  was  the  first national freight  transport  model that  took  into account  the  effect  of  logistics choices  on freight flows. In 2009, the Dutch MoT chose to invest in a more simple and straightforward freight  transport  model  that  would  also  be  easier  to  maintain.  A  basic  freight  transport model was developed, called BASGOED (where BAS comes from basic and GOED from good). This model was developed in about a year, and should be able to answer the most pressing  policy  questions  of  the  MoT  (Significance  et  al.2010).  BASGOED  is  a  conventional four-step transport model, with only a limited number of zones and commodity types.
    \end{itemize}
    \item \citet{deJong2016TheLevel}: (READ THIS RUBEN)
    \begin{itemize}
        \item This paper has some great info on NGM and the type of analysis that is done
        \item \textbf{\color{black}Table 1 highlights that the model framework can be used to generate forecasts for freight transport (tonnes) for future scenarios. It also states that the models can be used for forecasting emissions. I do not agree. They only use it in the way that \citet{Pinchasik2020CrossingNordics} does.}
        \item Requirements \textit{"What are the appropriate scope and level of detail of the model?"}
        \item \textit{"The required model scope and level of detail depend strongly on the issues under investigation. For instance, policy studies require mostly aggregated outputs either at the national or the regional level, \textbf{sometimes it is not even needed to relate the results to transport networks. This commonly is the case of national studies for the medium or long run related for instance to emissions forecast}, tax revenues or the impact assessment of policy measures."} \textbf{Argue that the network is needed, as well as the dynamics. Emission reduction is amongst others connected to network infrastructure investments } \red{- I agree, but we should be a bit careful. From a strategic publication point of view, we only want to emphasize the fact that the network is necessary if we obtain results that differ from what would be expected from the cost data alone }
        \item I like the start of section 3.2. Use some of it.
        \item \textit{\color{black}"Most national freight transport models apply \textbf{static concepts of time}, e.g. by calculating freight transport for isolated points in time. In contrast, \textbf{new developments} in freight transport research focus on the \textbf{continuous representation of time} by using dynamic simulation. Hence, the temporal scope either defines certain points in time or beginning and end of the analysis together with information on the temporal resolution in between."} No references here! But I think they refer to these system dynamics type of models? \red{- Very interesting. We should check this out}
    \end{itemize}
    \item \citet{Meersman2016ChallengesModelling}:
    \begin{itemize}
        \item \textit{"For modelling possible future developments this implies major challenges as the impact of new technologies is difficult to estimate and integrate. Not only does it imply that data itself is not available for simulating the impact of innovations and changes. \textbf{With their given, mostly static structures, freight transport models currently don't include the impact of innovations on structures and interrelations with other parameters of the system.}"} \red{- yes, this is a good quote}
        \item OUTLOOK: \textit{"New requirements towards international freight transport models, in particular the \textbf{impact of new technologies}, societal and social changes, the impact of transport costs on international trade and transport structures, the impact of international \textbf{environmental policies}  as well as the impact of structural changes of transport routings;"} \note{- another good quote}
    \end{itemize}
    \item \citet{Meersman2019FreightFuture}:
    \begin{itemize}
        \item First paper that is critical of the developed transport models for some of the same reasons as we.
        \item \textit{"The traditional model-based approach is no longer capable of grasping developments in freight transport within an ever more rapidly changing world. Most models that have been used in the past to explain and predict the demand for freight transport did not devote sufficient consideration to structural, organisational and behavioural changes. Several important global developments that are taking place could have a structural effect on freight transport, with a number of consequences for modelling. This paper addresses several global developments in greater depth, along with their impact on freight transport."}
        \item \textit{"Most existing methods and models have difficulty coping with \textbf{structural changes and the uncertainties} with which we are confronted. \textbf{The fundamental problem} is that they assume that the characteristics of the agents and the flows in the transport system (e.g. logistics, market structures, spatial organisation, perceptions, trade patterns) will remain largely unchanged"} 
        \item \red{question: what do these authors do? how does that compare to what we do?}
    \end{itemize}
\end{itemize}}
\ppt{ADA models \citep{Ben-Akiva2013TheSystem} (used in e.g. NGM): modes/routes are determined by decisions on a disaggregated firm-level. \notesjb{First sketch seems to be proposed around 2004 in \cite{deJong2004NationalDevelopment}.} \red{I have a reference for this; (look up)}}
\ppt{(mention other specifics that align with this trend) \orange{list in \citet{deJong2013RecentEurope}}}
\ppt{These detailed models are nice for detailed analyses on a tactical level \orange{explain how these models are used in long-term scenario analysis now}} 
\ppt{We are critical of the way in which the transport models have been used for the purpose of decarbonization analyses.}
\ppt{\orange{If we want to cite some aspects related to decarbonization (e.g. modal shift) in these transport models, then refer to \citet{Tavasszy2011ModalAssessment, Pinchasik2020CrossingNordics,Maurer2008DevelopmentTransport,Yan2021Climate2050}  Can we also integrate \citet{Rosell2022ATransport} in the intro?}}



\pt{But on strategic level (plan far into the future), more high-level low-resolution models are needed}
\red{Include the references mentioned above here: \cite{Meersman2019FreightFuture,Meersman2016ChallengesModelling,deJong2016TheLevel}}
\ppt{Motivate: use quote from \cite{deJong2004NationalDevelopment}}
\ppt{Specific issue: new technologies. No detailed data available, lots of uncertainty, changing fleet over time}
\ppt{Current static models do not suffice}
\ppt{Calls for strategic, dynamic, stochastic, ``multi-technology'' model}
\ppt{}


\pt{This paper: develop a \textit{strategic} multimodal transport network model}
\ppt{Aim: make a model that is suitable for strategic planning}
\ppt{Use \textit{multimodal transport networks models} (used in STAN, etc. (add refs)) as basic framework}
\ppt{Main idea: combine mode/route choice using an aggregate-level cost minimization model}
\ppt{Extend this framework for our purposes: \notesjb{contributions: (I like to highlight those)}
\begin{itemize}
    \item {Dynamic model: plan into the future}
\item {New technologies: new fuels needed for decarbonization (so allow for different fuel types on each mode)} \notesjb{Note that existing works tend to focus on detailed vehicle \textit{types} (that have features that are relevant for logistics)}
\item {Stochastic model: development of technologies is uncertain }
\end{itemize}
}


\pt{We apply the model to Norway to gain insight into the question of how to decarbonize Norwegian freight transport sector. }
\ppt{(mention main results here)}


\pt{The remainder of this paper is organized as follows}
\ppt{...}


==> Notes/path_generation.tex <==
Here are some notes about the section on path generation:

\red{What is special (and perhaps new) in our model in terms of path generation:
\begin{enumerate}
    \item Generating paths for a \textbf{multimodal} network.
    \begin{itemize}
        \item Done before? Yes, at least in the NGM model. But maybe it hasn't been mentioned in the academic literature yet.
    \end{itemize}
    \item \textbf{Multiple fuels} using the same (modal) arc. This leads to different possible transport costs on the same arc, which should be taken into account.
    \begin{itemize}
        \item Done before? Don't know yet.
    \end{itemize}
    \item \textbf{Uncertainty} in the transport cost. This again leads to different possible transport costs on the same arc.
    \begin{itemize}
        \item Done before? Don't know yet.
    \end{itemize}
\end{enumerate}}

\blue{
\textbf{Literature:}
\begin{itemize}
    \item \cite{Guelat1990AFlows}: Original multimodal transport model formulation. Introduces an arc-path-flow formulation. No real motivation is given for the paths, except ``notational convenience''
    \item \cite{Crainic2007ChapterTransportation} repeat the formulation but don't say much about the relevance of paths or path generation. Only that paths model what modes can be used by different products.
    \item \cite{Crainic1997PlanningTransportation} also don't say much about it.
    \item \cite{Crainic2008NationalInstruments}: same.
    \item \cite{Crainic1997PlanningTransportation}: path-formulation has the benefit that some constraints can be incorporated in the path definitions, they can handle non-linear route costs, may open interesting algorithmic perspectives (here they refer to \cite{Crainic2000ADesign}, which propose a column generation approach, where new paths are iteratively generated). 
    \item \cite{VanRiessen2013ImpactNetworks}: intermodal contrainer transportation network design. They use a path generation algorithm based on a list of requirements (max. 3 legs, max 10\% detour, certain modal requirements, max. 8 days). All paths are generated using the $k$-shortest path algorithm by Yen (1974). Then all paths not satisfying the conditions are removed.
    \item \cite{Zhang2008ApplicationNetwork}: intermodal multiproduct freight network simulation-assignment model (applied to intermodal rail network). Path generation for each mode and product type (``because each product type may experience different generalized cost on the same physical and service path'') using an extended intermodal least-cost path algorithm by \cite{Zhou2008DynamicManagement} (which basically just means: generate the $k$ shortest paths). \\
    Note that the fact that the path generation is repeated for every commodity (and mode? I don't understand that part) is analogous to our setting with multiple fuels/scenarios.
    \item Some papers in related fields (especially operational models with time windows) use \textit{column generation} approaches. Here, paths are iteratively generated during the course of the solution algorithm. In contrast, we \textit{first} generate a set of paths, and then solve the model (so we do not guarantee to include the optimal paths). Some references in this direction are: \cite{Moccia2011ModelingServices} for an example and \cite{PfetschLectureVerkehr} for a theoretical background.
    \item \cite{FebbraroHEURISTICSYSTEM} develop a shortest path heuristic in a multimodal transport network. It is an adaptation of Dijkstra's algorithm that takes different modes into account. 
    \item \cite{deJong2013Method3}: In NGM, the procedure BuildChain is used. It generates a multimodal path for every mode-combination from a pre-specified list. The main idea is to first generate unimodal shortest paths and then generate multi-modal shortest paths by finding the optimal transfer node. It cannot be used to find second-best paths. \\
    We use an adapted version of this method.
\end{itemize}
}



==> Notes/scope.tex <==
{\color{blue}
\begin{enumerate}
    \item {Intro}. 
    \begin{itemize}
        \item In this section we outline the scope of the model that we want to develop.
        \item What do we mean by scope? Boundaries of the model?
        \item Recap: what is the purpose of the model
        \item introduce multimodal freight transport approach on an aggregated level
    \end{itemize}
    \item National freight transport modeling
    \begin{itemize}
        \item Based on four step procedure. 
        \item Given our requirements, no need for structural changes in step 1 and 2. 
        \item We present an multimodal freight transport model that integrates step 3 and 4.
    \end{itemize}
    \item Spatial resolution
    \begin{itemize}
        \item why do we need a network -> Emission reduction is amongst others connected to network infrastructure investments
        \item large zones (counties) nationally, represented by big cities
        \item even larger zones internationally (how is this represented?)
        \item long-distance transport (>..km). No first-mile / last-mile. Assume this is done by electrified trucks.
        \item (geen wiskundige termen zoals node/graph)
    \end{itemize}
    \item Temporal resolution
    \begin{itemize}
        \item multi-year time steps?
    \end{itemize}
    \item Some specific elements
    \begin{itemize}
        \item what are modes (class of vehicle using the same infrastructure)
        \item what are fuels
        \item given a product group, we assume there is a representative vehicle with specific costs, capacities and emission factors.
        \item demand for transport on aggregated level (trade flow instead of physical flow) %trade flow (goods) vs. physical transport flow (vehicles) MOVE
    \end{itemize}
    \item Investments and capacities
    \begin{itemize}
        \item assume no capacity limits on road and sea
        \item we focus on aggregate capacities?
    \end{itemize}
    \item What should the model be doing?
    \begin{itemize}
        \item decide investments and the flow of transport through the network in terms of routes, modes and fuels used (step 3 and 4) 
        \item This is mainly done based on generalized transport costs. This includes ..... AND emission constraint
        \item \red{investment costs include NPV of Maintenance costs -> task for AIM}
        \item \red{freight sector not included in emission trading system (ETS). What if? do not mention yet.}
    \end{itemize}
    
\end{enumerate}
}


\note{maybe use text from thesis}
